Data Augmentations for Improved (Large) Language Model Generalization

The reliance of text classifiers on spurious correlations can lead to poor generalization at deployment, raising concerns about their use in safety-critical domains such as healthcare. In this work, we propose to use counterfactual data augmentation, guided by knowledge of the causal structure of the data, to simulate interventions on spurious features and to learn more robust text classifiers. We show that this strategy is appropriate in prediction problems where the label is spuriously correlated with an attribute. Under the assumptions of such problems, we discuss the favorable sample complexity of counterfactual data augmentation, compared to importance re-weighting. Pragmatically, we match examples using auxiliary data, based on diff-in-diff methodology, and use a large language model (LLM) to represent a conditional probability of text. Through extensive experimentation on learning caregiver-invariant predictors of clinical diagnoses from medical narratives and on semi-synthetic data, we demonstrate that our method for simulating interventions improves out-of-distribution (OOD) accuracy compared to baseline invariant learning algorithms.

==> Figures/simple_graph_revision.tex <==
% \begin{figure}[h!]
%% Rough Figure
\centering
\includegraphics[scale=0.7]{Figures/ac_basic.drawio.pdf}
 \caption{Prediction problem with a spuriously correlated attribute.}
 
% $X$ is a high dimensional unstructured input (e.g. an embedding of raw text in $\sR^d$), $Y$ is a label and $C$ the attribute. Dashed red colored edge $C {\color{red}\leftrightarrow} Y$ marks an unstable association. Since we assume $X^*$ can be recovered from $X^*$, correlation between $Y$ and $C$ is only due to the unstable association.
%  We assume that all information about $Y$ unstable correlation is ``purely spurious" in the sense that there exists a latent $d^*$ dimensional sufficient statistic $X^*$ that is recoverable from $X$ and captures all relevant information about $Y$.
% \end{figure}

==> Figures/simple_graphs.tex <==
\begin{figure}[h!]
%% Rough Figure
\centering
\begin{subfigure}[b]{0.4\textwidth}
\centering
\includegraphics[scale=0.8]{Figures/ac_basic.drawio.pdf}
%   \tikz{
% % nodes
%  \node[latent,fill] (X) {$X$};%
% %  \node[latent,right=of X,xshift=0.5cm,fill] (U) {$U$}; %
% %  \node[circle,fill=yellow,above=of X,yshift=0.5cm,fill] (S) {$S$}; %
%  \node[latent,above right=of X,xshift=0.05cm,yshift=-0.2cm,fill] (Y) {$Y$}; %
%  \node[latent, rectangle,left=of Y,xshift=-0.8cm,fill, dashed] (C) {$C$}; %
%  % \node[latent,left=of C,xshift=0.2cm,fill, dashed] (E) {$E$}; %

% %  \draw (0,1.69) circle(.36cm);
% % plate
%  \plate [inner sep=.15cm,yshift=.15cm] {} {(X)(Y)} {}; %
%  % \plate [inner sep=.3cm,yshift=.1cm] {} {(X)(C)(Y)} {}; %
% % edges
%  \edge {C} {X}
%  % \edge {E} {C}
%  \edge {Y} {X}
%  \draw[<->, dash dot] (Y) to[out=90, in=90, distance=0.8cm] (C)
%  }



%  \tikz{
% % nodes
%  \node[latent,fill=black!20] (X) {$X$};%
% %  \node[latent,right=of X,xshift=0.5cm,fill] (U) {$U$}; %
% %  \node[circle,fill=yellow,above=of X,yshift=0.5cm,fill] (S) {$S$}; %
%  \node[latent, above right=of X, xshift=-0.5cm, yshift=0.5cm, fill=black!20] (Y) {$Y$}; %
%  \node[latent, left=of Y, xshift=0.2cm, fill=black!20] (C) {$C$}; %
%  \node[latent, below=of Y, yshift=0.7cm, fill] (Xsuff) {$X^*$};
%  % \node[latent,left=of C,xshift=0.2cm,fill, dashed] (E) {$E$}; %

% %  \draw (0,1.69) circle(.36cm);
% % plate
% %  \plate [inner sep=.15cm,yshift=.15cm] {} {(X)(Y)(Xs)(Xsuff)} {}; %
%  % \plate [inner sep=.3cm,yshift=.1cm] {} {(X)(C)(Y)} {}; %
% % edges
%  \edge {C} {X}
%  % \edge {E} {C}
%  \edge {Y} {Xsuff}
%  \edge {Xsuff} {X}
%  \draw[<->, dash dot] (Y) to[out=90, in=90, distance=0.8cm] (C)
%  }
 
 \caption{}
 \label{fig:dgp_purely_spu_ac}
\end{subfigure}
\begin{subfigure}[b]{0.4\textwidth}
\centering
    \includegraphics[scale=0.8]{Figures/d_in_d_mednotes.drawio.pdf}
%   \tikz{
% % nodes
%  \node[latent,fill] (X) {$X$};%
% %  \node[latent,right=of X,xshift=0.5cm,fill] (U) {$U$}; %
% %  \node[circle,fill=yellow,above=of X,yshift=0.5cm,fill] (S) {$S$}; %
%  \node[latent,above right=of X,xshift=-0.2cm,yshift=0.5cm,fill] (Y) {$Y$}; %
%  \node[latent,rectangle,left=of Y,xshift=-1.25cm,fill, dashed] (C) {$C$}; %
%  \node[latent,below=of C, xshift=1.0cm, yshift=0.7cm, fill=black!20] (Xs) {$X_s$};
%  \node[latent,below=of Y, yshift=0.7cm, fill=black!20] (Xsuff) {$X^*$};
%  % \node[latent,left=of C,xshift=0.2cm,fill, dashed] (E) {$E$}; %

% %  \draw (0,1.69) circle(.36cm);
% % plate
%  \plate [inner sep=.15cm,yshift=.15cm] {} {(X)(Y)(Xs)(Xsuff)} {}; %
%  % \plate [inner sep=.3cm,yshift=.1cm] {} {(X)(C)(Y)} {}; %
% % edges
%  \edge {C} {Xs}
%  % \edge {E} {C}
%  \edge {Y} {Xsuff}
%  \edge {Xs} {X}
%  \edge {Xsuff} {X}
%  \draw[<->, dash dot] (Y) to[out=90, in=90, distance=0.8cm] (C)
%  }
 \caption{}
 \label{fig:dgp_dind}
\end{subfigure}
 %% Detailed Figure
% \begin{subfigure}[b]{0.45\textwidth}
%   \centering
% \centering
%   \tikz{
% % nodes
%  \node[latent,fill] (X) {$X$};%
% %  \node[latent,right=of X,xshift=0.5cm,fill] (U) {$U$}; %
%  \node[latent,above right=of X,xshift=0.3cm,yshift=-0.3cm,fill] (Y) {$Y$}; %
%  \node[latent,above=of X,yshift=-0.7cm,fill] (S) {$S$}; %
%  \node[latent,left=of X,xshift=-0.3cm,fill] (C) {$C$}; %
%  \node[latent,left=of C,xshift=0.2cm,fill, dashed] (E) {$E$}; %

% %  \draw (0,1.69) circle(.36cm);
% % plate
%  \plate [inner sep=.15cm,yshift=.15cm] {} {(X)(Y)} {}; %
%  \plate [inner sep=.3cm,yshift=.1cm] {} {(X)(S)(C)(Y)} {}; %
% % edges
%  \edge {C} {X}
%  \edge {E} {C}
% %  \edge {E} {S}
%  \edge {Y} {X}
%  \edge {Y} {S}
%  \edge {S} {C}
%  \edge {S} {X}
%  \draw[->] (E) to[out=45, in=170, distance=0.5cm] (S)
% %  \draw[<->, dash dot] (Y) to[out=180, in=30, distance=0.8cm] (C)
%  }
%  \caption{}
%  \end{subfigure}
 
 \caption{\textbf{(a)} Anti-causal prediction problem with a spuriously correlated attribute. $X$ corresponds to a high-dimensional unstructured input (e.g. an embedding of raw text in $\sR^d$), $Y$ is a label and $C$ the attribute. A dashed red colored edge between $C$ and $Y$ marks an unstable association between the two, governed by unobserved factors. It is assumed that the unstable correlation is ``purely spurious" in the sense that there exists a latent $d^*$ dimensional sufficient statistic $X^*$ that is recoverable from $X$ and captures all relevant information about $Y$. \textbf{(b)} A causal graph that accommodates the use of a diff-in-diff estimator, e.g. as in our medical notes example. The difference in pre-treatment features $\rvx_{\text{pre}, i}, \rvx_{\text{pre}, j}$ for a pair of examples with the same pre-treatment attribute value, $c_{\text{pre}, i} = c_{\text{pre}, j}$, is used to account for the difference induced by attribute values $c_i \neq c_j$ to their features $\rvx_i, \rvx_j$ (from which we predict the label). Pairs $i,j$ are also matched according to meta-data $S$.
%  An unobserved factor, such as environment $E$ (corresponding to the hospital in our example) may change $P(C, Y)$, creating a disparity between conditioning and intervening on $C$. \yw{we might want to change the graph in (a) to have a dashed edge between $E$ and $Y$ instead of $C$ and $Y$}
}  
\end{figure}

==> Sections/backup_proof.tex <==
\begin{repdefinition}{def:prob_setting}
Consider random variables $X, X^*,Y,C$ taking on values in $\gX, \gX^*, [L], [K]$ respectively, that conform to the following generative process,
\begin{align} \label{eq:anti_causal_dgp}
    Y &= N_Y, \\
    C &= f_C(Y, N_{C}) \nonumber \\
    X^* &= f_{X^*}(Y, N_{X^*}), \nonumber \\
    % X_C = f_{X_C}(C, N_{X_C})
    X &= f_{X}(X^*, C, N_{X}). \nonumber
\end{align}
Here $N_Y, N_C, N_{X^*}, N_X$ are exogenous noise variables. Further consider an additional random variable $M$ taking on values in space $\gM$. An anti-causal prediction problem with a spuriously-correlated attribute is a set of probabilistic causal models, whose corresponding set of distributions with members $P(X, X^*, Y, C, M)$ have marginals $P(X, X^*, Y, C)$ that consist of all the distributions induced by interventions on $C$ in the structural equations of \cref{eq:anti_causal_dgp}. This amounts to the following set of distributions,
\begin{align*}
\gP = \left\{ P(X \mid X^*, C)P(X^* \mid Y)P(Y)\tilde{P}(C \mid Y) ~:~ \tilde{P}(C \mid Y=y)\in\Delta^{K-1} ~~ \forall y\in{[L]} \right\},
\end{align*}
where all distributions other than $\tilde{P}(C \mid Y)$ are fixed. Under the settings of this problem, a learner is provided with a set $\left\{ (\rvx_i, y_i, c_i) \right\}_{i=1}^{N}$ sampled i.i.d from $P_{\text{train}}\in{\gP}$.
\end{repdefinition}
% Consider a probabilistic causal model with endogenous random variables $X, X^*, Y, C, M$ and exogenous independent random variables \citep{peters2017elements}, where
% \begin{itemize}
%     \item $Y$ is $d$-separated from $X$ by $X^*, C$.
%     \item $Y, X^*$ are not descendants of $C$.
%     \item $X$ is a leaf.
% \end{itemize}

% Where $X$ is a leaf (has no children in the graph), all active paths between $Y,X$ that do not go through $X^*$ must go through $C$
Our assumptions on this problem that enable risk-invariant prediction with a single model $h(\rvx) = \mathrm{arg}\max_{y\in{[L]}} P_{\bot}(Y=y \mid X=\rvx)$ are given below.
\begin{assumption}
For an anti-causal prediction problem with a spuriously correlated attribute, we assume that $X^* = e(X)$ a.e. for some $e:\gX \rightarrow \gX^*$.
\end{assumption}
\begin{replemma}{lem:unconfounded_opt}
For the prediction problem in \cref{def:prob_setting}, the Bayes optimal classifier under the unconfounded distribution $P_\bot\in{\gP}$ where $C$ is uniformly distributed and independent of $Y$ is $h^*(\rvx) = \mathrm{arg}\max_{y\in{[K]}} P_\bot(Y=y \mid X^*=e(\rvx))$. It is a minimizer of $\min_{h:\gX\rightarrow [L] }\max_{P\in{\gP}}{\gR^{\ell_{01}}_{P}(h)}$ and $\gR^{\ell_{01}}_{P}(h^*)=\gR^{\ell_{01}}_{P_{\bot}}(h^*)$ for all $P\in{\gP}$.
\end{replemma}
\begin{proof}
    Assume $P_{\text{train}}(X, X^*, Y, C)$ is induced by a causal model with mechanism $f_C(Y, N_C)$.
    We will show that any hypothesis satisfying $h(X)=g\circ e(X)$ for some $g:\gX^*\rightarrow \gY$ (i.e. that only depends on $X^*$) achieves the same risk over all $P\in{\gP}$. To this end note that for such a hypothesis we have,
    \begin{align*}
        R^{\ell_{01}}_{P_{\text{train}}}(h) &= \int{ \ell_{01}(h(X), Y)P(X \mid C, X^*)P(X^* \mid Y)P(Y)P_{\text{train}}(C\mid Y) dX^*dXdYdC} \\ 
        &= \int{ \ell_{01}(g\circ e(X), Y)P(X \mid C, X^*)P(X^* \mid Y)P(Y)P_{\text{train}}(C\mid Y) dX^*dXdYdC} \\
        &= \int{ \ell_{01}(g(X^*), Y)P(X \mid C, X^*)P(X^* \mid Y)P(Y)P_{\text{train}}(C\mid Y) dX^*dXdYdC} \\ 
        &= \int{ \ell_{01}(g(X^*), Y)P(X^*, Y) dX^*dY}.
        %\E_{\rvx,y\sim P_{train}}{\left[ \ell_{01}(h(X), Y) \right]}
    \end{align*}
    Now consider any distribution $\tilde{P}$ that is induced by an intervention that replaces the mechanism $f_C$ in $P_{\text{train}}$ by another function $\tilde{f}_C(Y, N_C)$ or a fixed value $c$, we have that $\tilde{P}(X^*, Y) = P_{\text{train}}(X^*, Y)$ since $X^*, Y$ are not descendants of $C$. Hence if we repeat the derivation above for $R^{l_{01}}_{\tilde{P}}(h)$ we will obtain the same term (since $P(X^*, Y)$ are fixed regardless of the intervention applied in $\tilde{P}$, as argued earlier), and we may conclude $R^{\ell_{01}}_{P_{\text{train}}}(h)=R^{\ell_{01}}_{\tilde{P}}(h)$.
    
    Next to show that the Bayes optimal classifier over $P_{\bot}$ is the min-max optimal classifier w.r.t $\gP$. Consider the interventional distribution where $C$ is set to some fixed value $c\in{[K]}$, i.e. $P(X, X^*, Y \mid do(C=c))$. Under the graph we obtain from this intervention, $Y$ is $d$-separated from $X$ given $X^*$. Hence,
    \begin{align*}
    P(Y \mid X=\rvx, do(C=c)) &= \int_{X^*} P(Y \mid X^*, X=\rvx, do(C=c))P(X^* \mid X=\rvx, do(C=c))dX^* \\ 
    &= P(Y \mid X^*=e(\rvx), X=\rvx, do(C=c)) \\
    &= P(Y \mid X^*=e(\rvx), do(C=c)),
    \end{align*}
    where the first equality holds since $X^*=e(X)$ and the second from $d$-separation. Hence the Bayes optimal classifier under $P(Y, X \mid do(C=c))$ is $h^*(\rvx) = g\circ e(\rvx) = \mathrm{arg}\max_{y\in{[L]}}{P(Y=y \mid e(\rvx), do(C=c))}$. As argued earlier, since $Y, X^*$ are non-descendants of $C$, it holds that $P(Y \mid e(X), do(C=c))$ is fixed across all $c\in{[K]}$.
    Hence $h^*(\rvx)$ is the Bayes optimal classifier for all such interventional distributions and also for
    $P_{\bot}(X, Y) = \frac{1}{K}\sum_{c\in{[K]}}{P(X, Y \mid do(C=c))}$, and from our earlier discussion it is risk-invariant, i.e. $R^{\ell_{01}}_{P_{\bot}}(h^*) = R^{\ell_{01}}_{P}(h^*)$ for all $P\in{\gP}$, which also means $\max_{p\in{\gP}}{R^{\ell_{01}}_{P}(h^*)} = R^{\ell_{01}}_{P_{\bot}}(h^*)$. It is the min-max optimal classifier w.r.t $\gP$ since any $h \neq h^*$ will have $\max_{p\in{\gP}}{R^{\ell_{01}}_{P}(h)} \geq R^{\ell_{01}}_{P_{\bot}}(h) \geq R^{\ell_{01}}_{P_{\bot}}(h^*)$.
\end{proof}

==> Sections/graphs_drawing.tex <==
\begin{figure}[h!]
%% Rough Figure
\centering
\begin{subfigure}[b]{0.45\textwidth}
\centering
  \tikz{
% nodes
 \node[latent,fill] (X) {$X$};%
%  \node[latent,right=of X,xshift=0.5cm,fill] (U) {$U$}; %
%  \node[circle,fill=yellow,above=of X,yshift=0.5cm,fill] (S) {$S$}; %
 \node[latent,above right=of X,xshift=0.2cm,yshift=-0.2cm,fill] (Y) {$Y$}; %
 \node[latent,left=of X,xshift=-0.3cm,fill] (C) {$C$}; %
 \node[latent,left=of C,xshift=0.2cm,fill, dashed] (E) {$E$}; %

%  \draw (0,1.69) circle(.36cm);
% plate
 \plate [inner sep=.15cm,yshift=.15cm] {} {(X)(C)} {}; %
 \plate [inner sep=.3cm,yshift=.1cm] {} {(X)(C)(Y)} {}; %
% edges
 \edge {C} {X}
 \edge {E} {C}
 \edge {Y} {X}
 \draw[<->, dash dot] (Y) to[out=180, in=30, distance=0.8cm] (C)
 }
 \caption{}
 \end{subfigure}
 %% Detailed Figure
\begin{subfigure}[b]{0.45\textwidth}
  \centering
\centering
  \tikz{
% nodes
 \node[latent,fill] (X) {$X$};%
%  \node[latent,right=of X,xshift=0.5cm,fill] (U) {$U$}; %
 \node[latent,above right=of X,xshift=0.3cm,yshift=-0.3cm,fill] (Y) {$Y$}; %
 \node[latent,above=of X,yshift=-0.7cm,fill] (S) {$S$}; %
 \node[latent,left=of X,xshift=-0.3cm,fill] (C) {$C$}; %
 \node[latent,left=of C,xshift=0.2cm,fill, dashed] (E) {$E$}; %

%  \draw (0,1.69) circle(.36cm);
% plate
 \plate [inner sep=.15cm,yshift=.15cm] {} {(X)(S)(C)} {}; %
 \plate [inner sep=.3cm,yshift=.1cm] {} {(X)(S)(C)(Y)} {}; %
% edges
 \edge {C} {X}
 \edge {E} {C}
%  \edge {E} {S}
 \edge {Y} {X}
 \edge {Y} {S}
 \edge {S} {C}
 \edge {S} {X}
 \draw[->] (E) to[out=45, in=170, distance=0.5cm] (S)
%  \draw[<->, dash dot] (Y) to[out=180, in=30, distance=0.8cm] (C)
 }
 \caption{}
 \end{subfigure}
 
 \caption{(a) Anti-causal prediction problem, where $X$ corresponds to a high-dimensional unstructured input (e.g. an embedding of raw text in $\sR^d$). $Y$ is a label, in our example this is the diagnosis of the patient, and $C$ a nuisance such as the identity of the caretaker that wrote a medical note. An unobserved factor, such as environment $E$ (corresponding to the hospital in our example) may change $P(C, Y)$, creating a disparity between conditioning and intervening on $C$. \yw{we might want to change the graph in (a) to have a dashed edge between $E$ and $Y$ instead of $C$ and $Y$}
%  Causal graphical model describing how clinical narratives ($X$, in \textcolor{blue}{blue}) are generated in a hospital. A patient's condition ($y$, in \textcolor{red}{red}) affects its state ($S$, in \textcolor{yellow}{yellow}) that is observed through noisy lab results, and $U$ information that is unobserved through lab results but is visible to the doctor (e.g. "patient is pale"). The patient's state in turn affects the choice of caregivers ($C$, in \textcolor{yellow}{yellow}). The choice of caregivers is also affected by the hospital, or environment ($E$). $S,U,C$ all generate the information written in the clinical narrative $X$ and are generated at each doctor's visit.
 }  \label{fig:dgp_basic_ac}
\end{figure}
